UIFace: Unleashing Inherent Model Capabilities to Enhance Intra-Class Diversity in Synthetic Face Recognition

Face recognition (FR) stands as one of the most crucial applications in computer vision. The accuracy of FR models has significantly improved in recent years due to the availability of large-scale human face datasets. However, directly using these datasets can inevitably lead to privacy and legal problems. Generating synthetic data to train FR models is a feasible solution to circumvent these issues. While existing synthetic-based face recognition methods have made significant progress in generating identity-preserving images, they are severely plagued by context overfitting, resulting in a lack of intra-class diversity of generated images and poor face recognition performance. In this paper, we propose a framework to Unleash Inherent capability of the model to enhance intra-class diversity for synthetic face recognition, shortened as UIFace. Our framework first trains a diffusion model that can perform sampling conditioned on either identity contexts or a learnable empty context. The former generates identity-preserving images but lacks variations, while the latter exploits the model's intrinsic ability to synthesize intra-class-diversified images but with random identities. Then we adopt a novel two-stage sampling strategy during inference to fully leverage the strengths of both types of contexts, resulting in images that are diverse as well as identitypreserving. Moreover, an attention injection module is introduced to further augment the intra-class variations by utilizing attention maps from the empty context to guide the sampling process in ID-conditioned generation. Experiments show that our method significantly surpasses previous approaches with even less training data and half the size of synthetic dataset. The proposed UIFace even achieves comparable performance with FR models trained on real datasets when we further increase the number of synthetic identities.

==> table/table3.tex <==
\begin{table}[htbp]
    \caption{\textbf{
        The LPIPS, Improved Recall and final face recognition accuracy of synthetic datasets under different settings.}
        }
        \vspace{4pt}
    \label{tab:diversity}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|l|l|l|l|l|l}
    \hline
    Method                      & Num of imgs (IDs $\times$ imgs/ID)            & \textbf{LFW}        & \textbf{CFP-FP}        & \textbf{CPLFW}         & \textbf{AGEDB}      & \textbf{CALFW}  & \textbf{Average}     \\ \hline
    CASIA-Real                  & \textasciitilde0.5M(~10.5K $\times$ 47)                     & 99.43             & 97.27          & 90.18             & 94.78        & 93.58  & 95.05     \\
    baseline                    & 0.5M(10k $\times$ 50)                         & 98.88             & 92.4           & 87.92             & 88.67        & 91.15  & 91.80    \\
    baseline + 2-stage          & 0.5M(10k $\times$ 50)                         & 99.05             & 94.13          & 88.93              & 89.92        & 91.48 & 92.70         \\
    baseline + attn             & 0.5M(10k $\times$ 50)                         & 99.17             & 92.73          & 88.12              & 89.47       & 91.75  & 92.25          \\ 
    baseline + 2-stage + attn   & 0.5M(10k $\times$ 50)                         & \textbf{99.27}        & \textbf{94.29}            & \textbf{89.58}     & \textbf{90.95}        & \textbf{92.25}  & \textbf{93.27}   \\\hline
    \end{tabular}
    }
\end{table}

==> table/table4.tex <==
\begin{table}[h]
    \caption{\textbf{
        Comparisons with state-of-the-art synthetic-based face recognition methods on Real-Syn performance gap.} We calculate performance gap between synthetic-based and real dataset-based methods as (REAL - SYN)/SYN.
        }
    \label{tab:gap}
    \centering
    \begin{tabular}{c|l|c|c}
    \hline
    Method     & Num of imgs (IDs $\times$ imgs/ID)         & Average     & Performance gap\\ \hline
    CASIA-Real                  & \textasciitilde0.5M(~10.5K $\times$ 47)       & 95.05  &\textbf{0.0}\%   \\\hline
    SynFace    & 0.5M(10k $\times$ 50)                      & 74.75      &27.2\%    \\
    DigiFace   & 0.5M(10k $\times$ 50)                      & 83.45      &13.9\%    \\
    DCFace     & 0.5M(10k $\times$ 50)                      & 89.56      &6.1\%      \\ 
    IDiff-Face & 0.5M(10k $\times$ 50)                      & 88.20      &7.8\% \\ 
    Arc2Face   & 0.5M(10k $\times$ 50)                      & 91.73      &3.6\%       \\ 
    UIFace (ours)       & 0.5M(10k $\times$ 50)                      & \textbf{93.27} &\textbf{1.9\%}   \\\hline
    DigiFace   & 1.2M(10k $\times$ 72 + 100k $\times$ 5)    & 86.37      &10.0\%   \\
    DCFace     & 1.2M(20k $\times$ 50 + 40k $\times$ 5)     & 91.21      &4.2\%    \\ 
    Arc2Face   & 1.2M(20k $\times$ 50 + 40k $\times$ 5)     & 93.14      &2.0\%    \\
    UIFace (ours)       & 1.0M(20k $\times$ 50)             & \textbf{94.06} &\textbf{1.1\%}\\ \hline
    UIFace (ours)       & 1.5M(30k $\times$ 50)             & \textbf{94.54} &\textbf{0.5\%}\\ \hline
    \end{tabular}
\end{table}
